One-Shot Generalization in Deep Generative Models

Humans have an impressive ability to reason about new concepts and experiences from just a single example. In particular, humans have an ability for one-shot generalization: an ability to encounter a new concept, understand its structure, and then be able to generate compelling alternative variations of the concept. We develop machine learning systems with this important capacity by developing new deep generative models, models that combine the representational power of deep learning with the inferential power of Bayesian reasoning. We develop a class of sequential generative models that are built on the principles of feedback and attention. These two characteristics lead to generative models that are among the state-of-the art in density estimation and image generation. We demonstrate the one-shot generalization ability of our models using three tasks: unconditional sampling, generating new exemplars of a given concept, and generating new exemplars of a family of concepts. In all cases our models are able to generate compelling and diverse samples---having seen new examples just once---providing an important class of general-purpose models for one-shot machine learning.

==> defns.tex <==
%dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi

\usepackage{subfigure}
\usepackage{epsfig}
\usepackage{amsmath,amsthm,amssymb}
\usepackage{url}
\usepackage{rotating}

\def\Section {\S}
%allows you to replace the rather long "Section 5" by §5 when you use \Section 5. 

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }
 
%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}

%% a trick that makes the title take up less space for many style files (but not article)
%\addtolength{\titlebox}{-1.8cm}

%% densify spacing in bibliographies
\newcommand{\bibfix}{%    PUT \bibfix in file.bbl after first line
    \setlength{\parsep}{\parskip}%
    \setlength{\itemsep}{0cm}%
    \setlength{\topsep}{\parskip}%
    \setlength{\parskip}{0cm}%
    \setlength{\partopsep}{0cm}%
    \setlength{\listparindent}{\parindent}%
    \setlength{\labelwidth}{10pt}%
    \setlength{\labelsep}{0pt}%
    \setlength{\leftskip}{0pt}%
    \setlength{\leftmargin}{0pt}%
}

%% change margins
%\setlength{\textwidth}{7in}
%\setlength{\textheight}{8.75in}
%\setlength{\oddsidemargin}{-0.25in}
%\setlength{\evensidemargin}{-0.25in}
%\setlength{\headsep}{10pt}

%Use changebar.sty  to track changes.

%Saving space: see
%   http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html

%Page layout info:
%   http://amath.colorado.edu/documentation/LaTeX/reference/layout.html



%Latex
%\documentstyle[fleqn,psfig,epsfig]{article}
%\documentstyle[psfig]{article}
%\setlength{\textwidth}{6.5in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\textheight}{8.5in}
%\setlength{\headheight}{0in}
%\setlength{\headsep}{0in}
%\setlength{\parindent}{0in} % block style
%\setlength{\parskip}{0.3cm}

\newtheorem{thm}{Theorem}[section]
\newtheorem{corr}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}
\newenvironment{myproof}{{\bf Proof}}{}

\newcommand{\intersect}{\mbox{$\cap$}}
%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\mbox{$\frac{1}{2}$}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
%\newcommand{\defeq}{\mbox{$\stackrel{\rm def}{=}}$}
%\newcommand{\real}{{\rm I\hspace{-0.2em}R}}
\newcommand{\real}{\mbox{$\mathbb{R}$}}
\newcommand{\indep}{\mbox{$\perp$}}
\newcommand{\given}{\mbox{$|$}}
\newcommand{\ra}{\mbox{$\rightarrow$}}
\newcommand{\lra}{\mbox{$\leftrightarrow$}}
\newcommand{\Ra}{\mbox{$\Rightarrow$}}
\newcommand{\la}{\mbox{$\leftarrow$}}
\newcommand{\tr}{\mbox{$\mbox{tr}$}}
%\newcommand{\det}{\mbox{$\mbox{det}$}}

\newcommand{\rnd}[1]{\left(#1\right)}
\newcommand{\sqr}[1]{\left[#1\right]}
\newcommand{\crl}[1]{\left\{#1\right\}}
\newcommand{\ang}[1]{\langle#1\right\rangle}


\newcommand{\range}{\mbox{$\mbox{range}$}} 
\newcommand{\myspan}{\mbox{$\mbox{span}$}}
\newcommand{\nullspace}{\mbox{$\mbox{nullspace}$}}
\newcommand{\adj}{\mbox{$\mbox{adj}$}}
\newcommand{\nbd}{\mbox{$\mbox{nbd}$}}





\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\mbox{Discrete}}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{\mbox{${\cal N}$}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{\mbox{$NI\chi^2$}}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{\mbox{$p$}}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{\mbox{${\cal T}$}}
\newcommand{\student}{\mbox{${\cal T}$}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}


\newcommand{\define}[1]{{\bf #1}}

%\newcommand{\comment}[1]{}

\newcommand{\solnsrc}[1]{Source: #1}
\newcommand{\exsrc}[1]{(Source: #1)}

%\newenvironment{nam}[args]{begdef}{enddef}
%\newcommand{\includecodefig}[3]{
%\begin{figure}
%\noindent
%\hrulefill  
%\verbatiminput{#1}
%\noindent
%\hrulefill
%\noindent 
%}
%\caption{#2}
%\label{#3}
%\end{figure}
%}







%\newcommand{\includedudafig}[3]{
%\begin{figure}
%\centerline{\epsfig{file=c:/kmurphy/figures/duda/duda-#1.eps,height=#2}}
%\caption{#3 Source:
%\protect\cite{Duda01} Fig #1.}
%%Fig #1.}
%\label{fig:duda#1}
%\end{figure}
%}


%\newcommand{\keyword}[1]{{\bf #1}}
\newcommand{\keyword}[1]{{\bf #1}\index{keywords}{#1}}
\newcommand{\addtoindex}[1]{#1 \index{keywords}{#1}}
\newcommand{\keywordSpecial}[2]{{\bf #1}\index{keywords}{#2@#1}}
\newcommand{\bfidx}[1]{{\bf #1}}
\newcommand{\keywordDef}[1]{{\bf #1}\index{keywords}{#1|bfidx}}
%\newcommand{\keyworddef}[1]{{\bf #1}\index{keywords}{#1@{\bf #1}}}
\newcommand{\codename}[1]{{\tt #1}\index{code}{#1}}
\newcommand{\netlabname}[1]{{\tt #1}}
\newcommand{\Rcmd}[1]{{\tt #1}}
\newcommand{\matlabcmd}[1]{{\tt #1}}
\newcommand{\matlabscript}[1]{{\tt #1}}
\newcommand{\dataname}[1]{{\tt #1}}

%\newcommand{\dim}{\mbox{dim}}
\newcommand{\lse}{\mbox{lse}}
\newcommand{\softmax}{\calS}
%\newcommand{\softmax}{\mbox{softmax}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{\mbox{MATLAB}}
\newcommand{\MLABA}{\mbox{FML}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\myvec}[1]{\mbox{$\mathbf{#1}$}}
\newcommand{\myvecsym}[1]{\mbox{$\boldsymbol{#1}$}}

\newcommand{\vzero}{\mbox{$\myvecsym{0}$}}
\newcommand{\vone}{\mbox{$\myvecsym{1}$}}

\newcommand{\valpha}{\mbox{$\myvecsym{\alpha}$}}
\newcommand{\vbeta}{\mbox{$\myvecsym{\beta}$}}
\newcommand{\vchi}{\mbox{$\myvecsym{\chi}$}}
\newcommand{\vdelta}{\mbox{$\myvecsym{\delta}$}}
\newcommand{\vDelta}{\mbox{$\myvecsym{\Delta}$}}
\newcommand{\vepsilon}{\mbox{$\myvecsym{\epsilon}$}}
\newcommand{\veta}{\mbox{$\myvecsym{\eta}$}}
\newcommand{\vgamma}{\mbox{$\myvecsym{\gamma}$}}
\newcommand{\vmu}{\mbox{$\myvecsym{\mu}$}}
\newcommand{\vlambda}{\mbox{$\myvecsym{\lambda}$}}
\newcommand{\vLambda}{\mbox{$\myvecsym{\Lambda}$}}
\newcommand{\vLambdaBar}{\mbox{$\overline{\vLambda}$}}
\newcommand{\vphi}{\mbox{$\myvecsym{\phi}$}}
\newcommand{\vPhi}{\mbox{$\myvecsym{\Phi}$}}
\newcommand{\vpi}{\mbox{$\myvecsym{\pi}$}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\mbox{$\myvecsym{\Psi}$}}
\newcommand{\vtheta}{\mbox{$\myvecsym{\theta}$}}
\newcommand{\vTheta}{\mbox{$\myvecsym{\Theta}$}}
\newcommand{\vsigma}{\mbox{$\myvecsym{\sigma}$}}
\newcommand{\vSigma}{\mbox{$\myvecsym{\Sigma}$}}
\newcommand{\vOmega}{\mbox{$\myvecsym{\Omega}$}}
\newcommand{\vtau}{\mbox{$\myvecsym{\tau}$}}
\newcommand{\vxi}{\mbox{$\myvecsym{\xi}$}}

\newcommand{\va}{\mbox{$\myvec{a}$}}
\newcommand{\vb}{\mbox{$\myvec{b}$}}
\newcommand{\vc}{\mbox{$\myvec{c}$}}
\newcommand{\vd}{\mbox{$\myvec{d}$}}
\newcommand{\ve}{\mbox{$\myvec{e}$}}
\newcommand{\vf}{\mbox{$\myvec{f}$}}
\newcommand{\vg}{\mbox{$\myvec{g}$}}
\newcommand{\vh}{\mbox{$\myvec{h}$}}
\newcommand{\vj}{\mbox{$\myvec{j}$}}
\newcommand{\vk}{\mbox{$\myvec{k}$}}
\newcommand{\vm}{\mbox{$\myvec{m}$}}
\newcommand{\vn}{\mbox{$\myvec{n}$}}
\newcommand{\vp}{\mbox{$\myvec{p}$}}
\newcommand{\vq}{\mbox{$\myvec{q}$}}
\newcommand{\vr}{\mbox{$\myvec{r}$}}
\newcommand{\vs}{\mbox{$\myvec{s}$}}
\newcommand{\vt}{\mbox{$\myvec{t}$}}
\newcommand{\vu}{\mbox{$\myvec{u}$}}
\newcommand{\vv}{\mbox{$\myvec{v}$}}
\newcommand{\vw}{\mbox{$\myvec{w}$}}
\newcommand{\vws}{\mbox{$\vw_s$}}
\newcommand{\vwh}{\mbox{$\hat{\vw}$}}
\newcommand{\vx}{\mbox{$\myvec{x}$}}
\newcommand{\vxt}{\mbox{$\myvec{\tilde{x}}$}}
\newcommand{\vy}{\mbox{$\myvec{y}$}}
\newcommand{\vyt}{\mbox{$\myvec{\tilde{y}}$}}
\newcommand{\vz}{\mbox{$\myvec{z}$}}

\newcommand{\vA}{\mbox{$\myvec{A}$}}
\newcommand{\vB}{\mbox{$\myvec{B}$}}
\newcommand{\vC}{\mbox{$\myvec{C}$}}
\newcommand{\vD}{\mbox{$\myvec{D}$}}
\newcommand{\vE}{\mbox{$\myvec{E}$}}
\newcommand{\vF}{\mbox{$\myvec{F}$}}
\newcommand{\vG}{\mbox{$\myvec{G}$}}
\newcommand{\vH}{\mbox{$\myvec{H}$}}
\newcommand{\vI}{\mbox{$\myvec{I}$}}
\newcommand{\vJ}{\mbox{$\myvec{J}$}}
\newcommand{\vK}{\mbox{$\myvec{K}$}}
\newcommand{\vL}{\mbox{$\myvec{L}$}}
\newcommand{\vM}{\mbox{$\myvec{M}$}}
\newcommand{\vN}{\mbox{$\myvec{N}$}}
\newcommand{\vO}{\mbox{$\myvec{O}$}}
\newcommand{\vP}{\mbox{$\myvec{P}$}}
\newcommand{\vQ}{\mbox{$\myvec{Q}$}}
\newcommand{\vR}{\mbox{$\myvec{R}$}}
\newcommand{\vS}{\mbox{$\myvec{S}$}}
\newcommand{\vT}{\mbox{$\myvec{T}$}}
\newcommand{\vU}{\mbox{$\myvec{U}$}}
\newcommand{\vV}{\mbox{$\myvec{V}$}}
\newcommand{\vW}{\mbox{$\myvec{W}$}}
\newcommand{\vX}{\mbox{$\myvec{X}$}}
%\newcommand{\vXs}{\mbox{$\vX_{\vs}$}}
\newcommand{\vXs}{\mbox{$\vX_{s}$}}
\newcommand{\vXt}{\mbox{$\myvec{\tilde{X}}$}}
\newcommand{\vY}{\mbox{$\myvec{Y}$}}
\newcommand{\vZ}{\mbox{$\myvec{Z}$}}


\newcommand{\vxtest}{\mbox{$\myvec{x}_*$}}
\newcommand{\vytest}{\mbox{$\myvec{y}_*$}}


%\newcommand{\matlab}{{\bf MATLAB exercise}}
\newcommand{\matlabex}{(Matlab)}
%\newcommand{\matlabexx}{{\bf MATLAB exercise}\\}
\newcommand{\matlabexx}{}

\newcommand{\ftrue}{\mbox{$f_{true}$}}

\newcommand{\precw}{\mbox{$\lambda_{w}$}} % precision of weights (alpha)
\newcommand{\precy}{\mbox{$\lambda_{y}$}} % precision of y (beta)
\newcommand{\fbar}{\mbox{$\overline{f}$}}
\newcommand{\xbar}{\mbox{$\overline{x}$}}
\newcommand{\ybar}{\mbox{$\overline{y}$}}
\newcommand{\vxbar}{\mbox{$\overline{\vx}$}}
\newcommand{\vybar}{\mbox{$\overline{\vy}$}}
\newcommand{\Xbar}{\mbox{$\overline{X}$}}
\newcommand{\Ybar}{\mbox{$\overline{Y}$}}
\newcommand{\Jbar}{\mbox{$\overline{J}$}}
\newcommand{\Lbar}{\mbox{$\overline{L}$}}
\newcommand{\Tbar}{\mbox{$\overline{T}$}}

\newcommand{\htilde}{\mbox{$\tilde{h}$}}
\newcommand{\vhtilde}{\mbox{$\tilde{\vh}$}}
\newcommand{\Dtilde}{\mbox{$\tilde{D}$}}
\newcommand{\wtilde}{\mbox{$\tilde{w}$}}
\newcommand{\xtilde}{\mbox{$\tilde{x}$}}
\newcommand{\Xtilde}{\mbox{$\tilde{X}$}}
\newcommand{\ytilde}{\mbox{$\tilde{y}$}}
\newcommand{\Ytilde}{\mbox{$\tilde{Y}$}}
\newcommand{\vxtilde}{\mbox{$\tilde{\vx}$}}
\newcommand{\vytilde}{\mbox{$\tilde{\vy}$}}
\newcommand{\ztilde}{\mbox{$\tilde{\z}$}}
\newcommand{\vztilde}{\mbox{$\tilde{\vz}$}}
\newcommand{\vthetaMAP}{\mbox{$\hat{\vtheta}_{MAP}$}}
\newcommand{\vthetahat}{\mbox{$\hat{\vtheta}$}}
\newcommand{\thetahat}{\mbox{$\hat{\theta}$}}
\newcommand{\thetabar}{\mbox{$\overline{\theta}$}}
\newcommand{\vthetabar}{\mbox{$\overline{\vtheta}$}}
\newcommand{\pibar}{\mbox{$\overline{\pi}$}}
\newcommand{\vpibar}{\mbox{$\overline{\vpi}$}}



\newcommand{\sss}{\mbox{$s^2$}}
\newcommand{\vvv}{\mbox{$v$}}
\newcommand{\RSS}{\mbox{RSS}}

%\newcommand{\do}{\mbox{$\mbox{do}$}}


\newcommand{\vvec}{\mbox{$\mbox{vec}$}}
\newcommand{\dof}{\mbox{$\mbox{dof}$}}
\newcommand{\E}{\mbox{$E \;$}}
\newcommand{\Var}{\mbox{$\mbox{Var} \;$}}
\newcommand{\Std}{\mbox{$\mbox{Std} \;$}}
\newcommand{\Vvar}{\mbox{$\mbox{Var}$}}
%\newcommand{\mean}{\mbox{$\mbox{mean} \;$}}
%\newcommand{\mmean}{\mbox{$\mbox{mean}$}}
%\newcommand{\mode}{\mbox{$\mbox{Mode} \;$}}
%\newcommand{\Mode}{\mbox{$\mbox{Mode} \;$}}
%\newcommand{\Mmode}{\mbox{$\mbox{Mode}$}}
\newcommand{\Cov}{\mbox{$\mbox{Cov}$}}
%\newcommand{\diag}{\mbox{$\mbox{diag}$}}
\newcommand{\bias}{\mbox{$\mbox{bias}$}}
%\newcommand{\dim}{\mbox{$\mbox{dim}$}}
%\newcommand{\intersect}{\mbox{$\cap$}}
\newcommand{\union}{\mbox{$\cup$}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\NN}{\mbox{$N$}}
\newcommand{\NC}{\mbox{$N_C$}}
\newcommand{\ND}{\mbox{$N_D$}}
\newcommand{\NX}{\mbox{$N_X$}}
\newcommand{\NXi}{\mbox{$N_{X_i}$}}
\newcommand{\NY}{\mbox{$N_Y$}}

\newcommand{\nx}{\mbox{$n_x$}}
\newcommand{\ny}{\mbox{$n_y$}}
\newcommand{\nv}{\mbox{$n_v$}}
\newcommand{\nk}{\mbox{$n_k$}}
\newcommand{\nn}{\mbox{$n$}}

%\newcommand{\xdi}{\mbox{$x_{di}$}}
%\newcommand{\xji}{\mbox{$x_{ji}$}}
%\newcommand{\yi}{\mbox{$y_i$}}



\newcommand{\ki}{i}
\newcommand{\kj}{j}
\newcommand{\kk}{k}

\newcommand{\kC}{C}
\newcommand{\kc}{c}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calDx}{\mbox{${\cal D}_x$}}
\newcommand{\calE}{\mbox{${\cal E}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calG}{\mbox{${\cal G}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calHX}{\mbox{${\cal H}_X$}}
\newcommand{\calHy}{\mbox{${\cal H}_y$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\calK}{\mbox{${\cal K}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calMp}{\mbox{$\calM^+$}}
\newcommand{\calMm}{\mbox{$\calM^-$}}
\newcommand{\calMo}{\mbox{$\calM^o$}}
\newcommand{\Ctest}{\mbox{$C_*$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calSstar}{\mbox{$\calS_*$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}

\newcommand{\score}{\mbox{$\mbox{score}$}}
\newcommand{\scoreBIC}{\mbox{$\mbox{score-BIC}$}}
\newcommand{\scoreBICL}{\mbox{$\mbox{score-BIC-L1}$}}
\newcommand{\scoreL}{\mbox{$\mbox{score-L1}$}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{$\mbox{do}$}}
\newcommand{\data}{\calD}
\newcommand{\futuredata}{\tilde{\calD}}
%\newcommand{\data}{\mbox{$D$}}
\newcommand{\err}{\mbox{$\mbox{errr}$}}
\newcommand{\logit}{\mbox{$\mbox{logit}$}}
\newcommand{\sigmoid}{\mbox{$\sigma$}}

% We want to avoid name clashes with the exercise.sty package
%\newenvironment{myexercises}{\section{Exercises}}{}
\newenvironment{myexercises}{\section{Exercises}}{}
%\newenvironment{solutions}{\section*{Solutions} \begin{solutionsTag}}{\end{solutionsTag}}
%\newenvironment{solutions}{\section*{Solutions} \begin{comment}}{\end{comment}}
\newenvironment{mysolutions}{\section{Solutions}}{}
\newcommand{\myexercise}[1]{\vspace{0.5cm} \subsection{#1}}
\newcommand{\mysoln}[1]{\vspace{0.5cm} \subsection{#1}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

